Selective Activation of Aromatic C-H Bonds Catalyzed by Single Gold Atoms at Room Temperature

Selective activation and controlled functionalization of C-H bonds in organic molecules is one of the most desirable processes in synthetic chemistry. Despite progress in heterogeneous catalysis using metal surfaces, this goal remains challenging due to the stability of C-H bonds and their ubiquity in precursor molecules, hampering regioselectivity. Here, we examine the interaction between 9,10-dicyanoanthracene (DCA) molecules and Au adatoms on a Ag(111) surface at room temperature (RT). Characterization via low-temperature scanning tunneling microscopy, spectroscopy, and noncontact atomic force microscopy, supported by theoretical calculations, revealed the formation of organometallic DCA-Au-DCA dimers, where C atoms at the ends of the anthracene moieties are bonded covalently to single Au atoms. The formation of this organometallic compound is initiated by a regioselective cleaving of C-H bonds at RT. Hybrid quantum mechanics/molecular mechanics calculations show that this regioselective C-H bond cleaving is enabled by an intermediate metal-organic complex which significantly reduces the dissociation barrier of a specific C-H bond. Harnessing the catalytic activity of single metal atoms, this regioselective on-surface C-H activation reaction at RT offers promising routes for future synthesis of functional organic and organometallic materials.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
